Revisiting knowledge transfer for training object class detectors

We propose to revisit knowledge transfer for training object detectors on target classes from weakly supervised training images, helped by a set of source classes with bounding-box annotations. We present a unified knowledge transfer framework based on training a single neural network multi-class object detector over all source classes, organized in a semantic hierarchy. This generates proposals with scores at multiple levels in the hierarchy, which we use to explore knowledge transfer over a broad range of generality, ranging from class-specific (bicycle to motorbike) to class-generic (objectness to any class). Experiments on the 200 object classes in the ILSVRC 2013 detection dataset show that our technique: (1) leads to much better performance on the target classes (70.3% CorLoc, 36.9% mAP) than a weakly supervised baseline which uses manually engineered objectness [11] (50.5% CorLoc, 25.4% mAP). (2) delivers target object detectors reaching 80% of the mAP of their fully supervised counterparts. (3) outperforms the best reported transfer learning results on this dataset (+41% CorLoc and +3% mAP over [18, 46], +16.2% mAP over [32]). Moreover, we also carry out several across-dataset knowledge transfer experiments [27, 24, 35] and find that (4) our technique outperforms the weakly supervised baseline in all dataset pairs by 1.5x-1.9x, establishing its general applicability.

==> related_work.tex <==
\section{Related Work}

\mypartop{Weakly Supervised Object Detection.}

Many works address weakly supervised object
detection~\cite{bilen14bmvc,bilen15cvpr,bilen16cvpr,cinbis16pami,deselaers10eccv,russakovsky12eccv,siva11iccv,song14icml,song14nips,wang15tip}.
In most of these cases the problem is cast as a Multiple Instance Learning
problem~\cite{bilen14bmvc,bilen15cvpr,cinbis16pami,deselaers10eccv,russakovsky12eccv,siva11iccv,song14icml,song14nips}:
Each image is represented as a bag of windows, where windows are generally obtained using proposal
generation mechanisms~\cite{alexe10cvpr,dollar14eccv,uijlings13ijcv}. Given a target class, for
every positive image there is at least on correct window. For every negative image, all windows are
negative. The goal is to select those windows from the positive images to train a good detector.
This is done in an iterative fashion: (A) given a detector, apply this to the positive images to
obtain the highest scored window in each image. (B) Use the highest scored windows from (A) as
positive examples and re-train the object detector.


in this scenario. Perhaps the first
work was by Guillaumin and Ferrari~\cite{guillaumin12cvpr} who performed knowledge transfer for
object detection in ImageNet, exploiting the label-hierarchy of ImageNet. More recently, Hoffman et
al.~\cite{haha} proposed LSDA, where they used a classification network, and adapted the
weights of the final classification layer for detection, RCNN-style. There was also a follow-up.

[4, 5, 9, 12, 42, 47, 48, 49, 60].

